Towards Understanding Fairness and its Composition in Ensemble Machine Learning

Machine Learning (ML) software has been widely adopted in modern society, with reported fairness implications for minority groups based on race, sex, age, etc. Many recent works have proposed methods to measure and mitigate algorithmic bias in ML models. The existing approaches focus on single classifier-based ML models. However, real-world ML models are often composed of multiple independent or dependent learners in an ensemble (e.g., Random Forest), where the fairness composes in a non-trivial way. How does fairness compose in ensembles? What are the fairness impacts of the learners on the ultimate fairness of the ensemble? Can fair learners result in an unfair ensemble? Furthermore, studies have shown that hyperparameters influence the fairness of ML models. Ensemble hyperparameters are more complex since they affect how learners are combined in different categories of ensembles. Understanding the impact of ensemble hyperparameters on fairness will help programmers design fair ensembles. Today, we do not understand these fully for different ensemble algorithms. In this paper, we comprehensively study popular real-world ensembles: bagging, boosting, stacking and voting. We have developed a benchmark of 168 ensemble models collected from Kaggle on four popular fairness datasets. We use existing fairness metrics to understand the composition of fairness. Our results show that ensembles can be designed to be fairer without using mitigation techniques. We also identify the interplay between fairness composition and data characteristics to guide fair ensemble design. Finally, our benchmark can be leveraged for further research on fair ensembles. To the best of our knowledge, this is one of the first and largest studies on fairness composition in ensembles yet presented in the literature.

==> Draft.tex <==
\section{Fairness Composition in Ensembles} 

In this section, we evaluate the fairness of various type of ensemble models, divided into homogeneous and heterogeneous techniques, including bagging, boosting, stacking, etc. To ensure consistencies whilst comparing different metrics in the same table, Disparate Impact (DI) is converted to log scale. A value of 0 for any fairness metric suggests that there is no bias in the model. A positive value of a fairness metric suggests the model is biased against the privileged group whereas a negative value suggests bias against unprivileged group.


%Re-add

%\begin{mdframed}[leftmargin=1cm,
%    skipabove=0.2cm,    
%    linecolor=white,
%    backgroundcolor=gray!5,
%    linewidth=2pt,
%    roundcorner = 5pt,
%    innerleftmargin=1em,
%    innerrightmargin=1em,
%    innertopmargin=.75em,
%    innerbottommargin=.75em,
%    %userdefinedwidth=50em,
%]
%\noindent \textbf{RQ1. How fairness %composes in independent (parallel %ensemble) and dependent learners %(sequential ensemble)?} 
%\end{mdframed}



%\begin{mdframed}[leftmargin=1cm,
%    skipabove=0.2cm,    
%    linecolor=white,
%    backgroundcolor=gray!5,
%    linewidth=2pt,
%    roundcorner = 5pt,
%    innerleftmargin=1em,
%    innerrightmargin=1em,
%    innertopmargin=.75em,
%    innerbottommargin=.75em,
%    %userdefinedwidth=50em,
%]
%\noindent \textbf{RQ3. How much ensemble combinatory function effects fairness and performance of Ensemble?} 
%\end{mdframed}

%Re-add

%\begin{mdframed}[leftmargin=1cm,
%    skipabove=0.2cm,    
%   linecolor=white,
%    backgroundcolor=gray!5,
%    linewidth=2pt,
%    roundcorner = 5pt,
%    innerleftmargin=1em,
%    innerrightmargin=1em,
%    innertopmargin=.75em,
%    innerbottommargin=.75em,
%    %userdefinedwidth=50em,
%]
%\noindent \textbf{RQ2. Does the choice of combination methods improve %or worsen fairness?} 
%\end{mdframed}


%\begin{mdframed}[leftmargin=1cm,
%    skipabove=0.2cm,    
%    linecolor=white,
%    backgroundcolor=gray!5,
%    linewidth=2pt,
%    roundcorner = 5pt,
%    innerleftmargin=1em,
%    innerrightmargin=1em,
%    innertopmargin=.75em,
%    innerbottommargin=.75em,
%    %userdefinedwidth=50em,
%]
%\noindent \textbf{RQ1. How the homogeneity of the ensemble models affect fairness composition?} 
%\end{mdframed}


\textbf{Finding 1:}
\textbf{Boosting}


\textit{Dropout can improve fairness in larger datasets.} Vinayak and Gilad-Bachrach \cite{rashmi2015dart} proposed DART, a dropout technique derived from deep neural networks, for boosted trees. An ensemble of boosted regression trees are known for delivering high quality performances but they suffer from over-specification i.e. the trees added at the end have little contribution to the final result. DART alleviates this problem by introducing dropouts. This method works by selecting only a random subset of the already existing ensembles to compute the gradient that the next tree will fit. The number of trees dropped corresponds to the amount of regularization. In XGBoost, this rate is controlled by the parameter \textit{rate drop} with the range $[0,1]$. No trees are dropped on the lower end of this ratio, while on the higher extreme, all trees are dropped, which makes it similar to a Random Forest classifier. 




We investigate the efficacy of DART in reducing unfairness in boosting ensemble models by comparing its performance with the default XGBoost booster \textit{gbtree}. We analyze the performance of the dropout technique on all boosting models in each dataset and record the average change in each fairness metric. The average change is shown in Figure \ref{Dart:comparison}.


\begin{figure}[!htbp]
  \centering
  
    \includegraphics[width=\linewidth]{Figures/Dropout_figure.pdf}
    \caption{Change of performance and total bias when using DART (negative value denotes reduction in bias and accuracy performance}
    \label{Dart:comparison}
\end{figure}


Interestingly, our analysis shows that for larger datasets (Adult Census, Bank Marketing) we see an improvement across all fairness metrics except \textbf{Thiel Index}. However, for smaller datasets the exact opposite is seen. Our results suggest that using the dropout technique (DART) in boosting models can improve fairness performance at a comparable accuracy performance, in certain situations. Furthermore, it provides important insight into the affect of dropout on fairness, which can be further tuned to align with fairness goals, instead of accuracy.


\textbf{Finding2 :} \textbf{Randomness of feature split.}

One of the ways bagging models like Random Forest improve variance of the model is to induce randomness to the process of model building e.g. randomly selecting features. It has proven to be an effective way of reducing model bias (and hence fairness bias) when used in tandem with multiple learners and bagging. Building on this, Extra Trees introduces additional randomness by randomly selecting not only the subset of the features, but also randomly finding the splits for each feature and then finally taking the best split among those. Random Forest simply finds the best split for each feature. This begs the question, does randomness at feature splitting level cause Tree-based bagging models to be unfair?

To investigate this, we compare Random Forest and Extra Tree models in our benchmark. To ensure consistency in the rest of the parameter space and data split, we only choose those kernels that implement both Extra Trees and Random Forest. Bank Marketing and German Credit did not have any such kernels so we used the same kernel for both the models. For biased datasets such as Titanic and Adult (less biased), Extra Tree models with random splits were more biased compared to optimal splits (RF) Figure \ref{RF-ET:comparison}. This is especially interesting given that the model accuracy performance for models is similar or slightly lower, as can be expected when the optimal split is not chosen. However, it is important to note that for more fair models (BM and GC), randomness as little to no effect on fairness. In terms of bias mitigation methods, our results suggest randomness in the point of split might not be an effective way to tackle bias in decision-tree based models. 

\begin{figure}[!htbp]
  \centering
  
    \includegraphics[width=\linewidth]{Figures/Randomness of feature split.pdf}
    \caption{Change of performance and total bias when using DART (negative value denotes reduction in bias and accuracy performance}
    \label{RF-ET:comparison}
\end{figure}

\textbf{Finding 3: Soft Vs Hard Voting.}

A voting classifier is an ensemble method where the target label is assigned based on the probabilities each individual model within the classifier, assigns the chosen class variable. Voting classifier are of two types, Soft Voting and Hard Voting. In Hard Voting, the predicted target label is the label with majority of votes from each individual learner. Suppose we have 3 classifiers and they output (1,1,0) for the binary classification, then 1 is chosen as the final prediction due to majority voting. On the other hand, soft voting takes the average of the probabilities that each individual learner gives to each class e.g. (0.63, 0.51, 0.20) and (0.37, 0.49, 0.80) is the probabilities given by the 3 models in the voting classifiers for output class A,B respectively. Class A has an average probability 0.45 and Class B 0.55. Since, class B has a higher probability, we assign class B as the final prediction.

Here, we compare the effect of Soft Voting and Hard Voting on Fairness. We observe that for all fairness metrics except \textit{TI}, we see that soft voting outperforms hard voting in Titanic but vice-versa for the other 3 datasets, as shown in Table \ref{Soft vs Hard}. This difference in behavior can be attributed to Titanic's very biased dataset (SPD: ).
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \footnotesize
  \caption{Soft vs Hard Voting}
  \renewcommand{\tabcolsep}{1pt}
\resizebox{\columnwidth}{!}{    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multirow{8}{*}{\rotatebox[origin=c]{90}{Soft}} & & TM-VC1 & TM-VC2 & TM-VC3 & TM-VC4 & TM-VC5 & TM-VC6 & GC-VC1 & AC-VC1 & AC-VC2 & BM-VC1 & BM-VC2 \\
\cline{2-13}          & Acc & 0.853 & 0.821 & 0.835 & 0.839 & 0.810 & 0.813 & 0.757 & 0.828 & 0.826 & 0.915 & 0.937 \\
\cline{2-13}          & F1 & 0.808 & 0.784 & 0.756 & 0.796 & 0.738 & 0.731 & 0.517 & 0.507 & 0.560 & 0.569 & 0.938 \\
\cline{2-13}          & SPD & -0.764 & -0.798 & -0.737 & -0.778 & -0.772 & -0.585 & -0.093 & -0.095 & -0.140 & 0.174 & 0.253 \\
\cline{2-13}          & EOD & -0.579 & -0.701 & -0.441 & -0.674 & -0.625 & -0.482 & -0.026 & -0.074 & -0.143 & 0.144 & 0.019 \\
\cline{2-13}          & AOD & 0.538 & 0.631 & 0.534 & 0.581 & 0.629 & 0.376 & 0.107 & 0.048 & 0.097 & 0.127 & 0.044 \\
\cline{2-13}          & DI & -2.268 & -2.348 & -2.063 & -2.162 & -2.099 & -1.811 & -0.118 & -1.186 & -1.427 & 1.141 & 0.406 \\
\cline{2-13}          & TI & 0.119 & 0.146 & 0.098 & 0.116 & 0.124 & 0.155 & 0.116 & 0.176 & 0.168 & 0.067 & 0.036 \\ \cline{1-13}
    \multirow{7}{*}{\rotatebox[origin=c]{90}{Hard}} & Acc & 0.853 & 0.813 & 0.858 & 0.835 & 0.799 & 0.813 & 0.750 & 0.823 & 0.813 & 0.917 & 0.936 \\ 
\cline{2-13}          & F1    & 0.800 & 0.773 & 0.784 & 0.792 & 0.724 & 0.731 & 0.468 & 0.457 & 0.440 & 0.556 & 0.937 \\
\cline{2-13}          & SPD   & \cellcolor[rgb]{ .573,  .816,  .314}-0.746 & \cellcolor[rgb]{ .753,  0,  0}-0.826 & \cellcolor[rgb]{ .753,  0,  0}-0.793 & \cellcolor[rgb]{ .753,  0,  0}-0.788 & \cellcolor[rgb]{ .753,  0,  0}-0.783 & \cellcolor[rgb]{ .573,  .816,  .314}-0.568 & \cellcolor[rgb]{ .573,  .816,  .314}-0.062 & \cellcolor[rgb]{ .573,  .816,  .314}-0.072 & \cellcolor[rgb]{ .573,  .816,  .314}-0.067 & \cellcolor[rgb]{ .573,  .816,  .314}0.137 & \cellcolor[rgb]{ .753,  0,  0}0.262 \\
\cline{2-13}          & EOD   & \cellcolor[rgb]{ .753,  0,  0}-0.618 & \cellcolor[rgb]{ .753,  0,  0}-0.757 & \cellcolor[rgb]{ .753,  0,  0}-0.517 & \cellcolor[rgb]{ .753,  0,  0}-0.674 & \cellcolor[rgb]{ .753,  0,  0}-0.656 & \cellcolor[rgb]{ .573,  .816,  .314}-0.437 & \cellcolor[rgb]{ .753,  0,  0}-0.077 & \cellcolor[rgb]{ .573,  .816,  .314}-0.042 & \cellcolor[rgb]{ .573,  .816,  .314}-0.033 & \cellcolor[rgb]{ .573,  .816,  .314}0.142 & \cellcolor[rgb]{ .573,  .816,  .314}0.018 \\
\cline{2-13}          & AOD   & \cellcolor[rgb]{ .573,  .816,  .314}0.512 & \cellcolor[rgb]{ .753,  0,  0}0.688 & \cellcolor[rgb]{ .753,  0,  0}0.588 & \cellcolor[rgb]{ .753,  0,  0}0.603 & \cellcolor[rgb]{ .753,  0,  0}0.659 & \cellcolor[rgb]{ .573,  .816,  .314}0.353 & \cellcolor[rgb]{ .573,  .816,  .314}0.041 & \cellcolor[rgb]{ .573,  .816,  .314}0.026 & \cellcolor[rgb]{ .573,  .816,  .314}0.020 & \cellcolor[rgb]{ .573,  .816,  .314}0.105 & \cellcolor[rgb]{ .753,  0,  0}0.062 \\
\cline{2-13}          & DI    & \cellcolor[rgb]{ .753,  0,  0}-2.528 & \cellcolor[rgb]{ .753,  0,  0}-2.600 & \cellcolor[rgb]{ .753,  0,  0}-2.468 & \cellcolor[rgb]{ .753,  0,  0}-2.173 & \cellcolor[rgb]{ .753,  0,  0}-2.111 & \cellcolor[rgb]{ .573,  .816,  .314}-1.747 & \cellcolor[rgb]{ .573,  .816,  .314}-0.076 & \cellcolor[rgb]{ .573,  .816,  .314}-1.123 & \cellcolor[rgb]{ .573,  .816,  .314}-1.080 & \cellcolor[rgb]{ .573,  .816,  .314}1.065 & \cellcolor[rgb]{ .753,  0,  0}0.415 \\
\cline{2-13}          & TI    & \cellcolor[rgb]{ .753,  0,  0}0.131 & \cellcolor[rgb]{ .753,  0,  0}0.155 & \cellcolor[rgb]{ .573,  .816,  .314}0.089 & \cellcolor[rgb]{ .753,  0,  0}0.117 & \cellcolor[rgb]{ .753,  0,  0}0.130 & \cellcolor[rgb]{ .882,  .882,  .882}0.155 & \cellcolor[rgb]{ .573,  .816,  .314}0.105 & \cellcolor[rgb]{ .753,  0,  0}0.189 & \cellcolor[rgb]{ .753,  0,  0}0.203 & \cellcolor[rgb]{ .753,  0,  0}0.070 & \cellcolor[rgb]{ .753,  0,  0}0.036 \\
    \hline
    \end{tabular}}%
  \label{Soft vs Hard}%
\end{table}%

\textbf{Finding: Are voting ensembles guaranteed to be at least as fair as the individual learners?}

In homogeneous models, especially bagging, we have seen that the ensemble is guaranteed to be more fair than the most biased individual learner in the ensemble. However, does that claim hold for heterogeneous models? Are heterogeneous models guaranteed to outperform their individual classifiers? We find that this is not true always true. For example, TM-VC5 is a soft voting ensemble with 3 classifiers \textit{Logistc Regression (LR)}, \textit{Random Forest (RF)} and \textit{AdaBoost (ADB)}. The results for these individual classifiers along with the ensemble are reported in Table \ref{Voting-Guarantee}. We can see that in terms of \textit{SPD} and \textit{AOD}, the Voting ensemble actually performs worse than the most biased individual classifiers (\textit{LR} in this case). Recall from earlier that soft-voting takes the average of the probabilities for each class label (with the higher winning). Since the performance in Hard voting is even worse, we can conclude that the performance is not worse due to any single classifier. However, as seen in Table \ref{Voting-Guarantee}, this can be attributed to the fact that the ensemble has outperformed its individual classifiers, in terms of accuracy. In other words, this suggests that the number of correct but \textit{biased} predictions in the ensemble increases (both average of probabilities and majority voting), compared to the total sum of unique biased predictions from the individual classifiers. Upon further investigation, we could not specifically pinpoint responsibility to a single classifier rather than the combination of them. When we added further classifiers like XGBoost and Bagging Classifier, we saw the ensemble outperform significantly (SPD: -0.685 \& AOD: 0.518). Since there is no method to select classifiers before testing/validating the ensemble, we suggest using at-least 5 classifiers in the voting ensemble, which is the next odd number, to increase the diversity of the model pool and reduce chances of biased performance. We note that all the other Titanic models do not exhibit this phenomenon and have more than 3 individual classifiers which reduces the probability of stumbling upon such a combination of probabilities.

% Table generated by Excel2LaTeX from sheet 'Voting vs Individual Learner'
\begin{table}[htbp]
  \centering
  \caption{Performance of individual classifiers vs final voting ensemble TM-VC5}
    \begin{tabular}{|c|cccc|}
    \hline
    \multicolumn{1}{|c}{} & \multicolumn{1}{|c}{\textbf{LR}} & \textbf{RF} & \textbf{ADB} & \textbf{Voting} \\ \hline
    \textbf{Acc} & 0.795 & 0.787 & 0.761 & 0.810 \\
    \textbf{F1} & 0.718 & 0.698 & 0.686 & 0.738 \\
    \textbf{SPD} & -0.751 & -0.729 & -0.722 & -0.772 \\
    \textbf{EOD} & -0.671 & -0.671 & -0.671 & -0.625 \\
    \textbf{AOD} & 0.628 & 0.614 & 0.621 & 0.629 \\
    \textbf{DI} & -2.074 & -2.146 & -1.773 & -2.099 \\
    \textbf{TI} & 0.137 & 0.148 & 0.144 & 0.124 \\
    \hline
    \end{tabular}%
  \label{Voting-Guarantee}%
\end{table}%

\textbf{Finding: Odd number of classifiers in hard voting classifiers?}





\begin{mdframed}[leftmargin=1cm,
    skipabove=0.2cm,    
    linecolor=white,
    backgroundcolor=gray!5,
    linewidth=2pt,
    roundcorner = 5pt,
    innerleftmargin=1em,
    innerrightmargin=1em,
    innertopmargin=.75em,
    innerbottommargin=.75em,
    %userdefinedwidth=50em,
]
\noindent \textbf{RQ3. How does increasing or decreasing the number of weak learners affect fairness in ensemble learning?} 
\end{mdframed}

As discussed before, ensemble methods are mainly divided into homogeneous and heterogeneous models. \textit{Number of trees} or \textit{number of boosting rounds} is one of the most important hyper-parameters for homogeneous methods and refers to the total number of individual learners that make up the ensemble. To understand the composition of fairness, the effect of the \textit{number of trees/rounds} on fairness in Boosting and Bagging methods needs to be explored.In this section, we discuss the implication of number of inidividual learners on fairness.

\textbf{Boosting.} We analyze the boosting models (XGBoost, AdaBoost and Gradient Boosting) across the four datasets in our benchmark to investigate the effect of number of boosting rounds on fairness. We generate the fairness metrics and accuracy scores after each boosting round, and analyze the fairness performance across different models. We have found that given a biased dataset against a protected attribute, the number of weak boosting rounds overall has a positive affect on fairness performance metrics such as SPD, EOD and DI but negatively impacts AOD. For the datasets in our benchmark, the statistical parity difference (SPD) score for Titanic dataset is -0.553, which indicates a higher level of bias against male passengers. On the other hand, Adult, Bank Marketing and German Credit have a SPD score of -0.196303, 0.130428, -0.074801 respectively, that are much lower. To understand this better, let's take a look at Figure \ref{titanic_boosters} which shows the performance of boosting models for the Titanic dataset.

\begin{figure}[ht] 
\footnotesize
  %\begin{subfigure}[b]{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Titanic_Boosting_Estimators.pdf} 
    %\caption{Initial condition} 
  %\end{subfigure}%% 
  
  \caption{Performance of boosting models in the Titanic Dataset across boosting round (DI dropped for scaling) }
  \label{titanic_boosters} 
\end{figure}



We can see that for all of the different boosting models, except TM-ADB2, SPD, AOD, EOD improve as the boosting rounds proceed. This is due to the behavior of weak learners and the design of boosting models to improve upon the previous learner's incorrect predictions. Therefore, when a dataset is very biased against the protected attribute in an unbalanced dataset, the protected attribute is one of the strongest feature in the weak learner. Since most of the predictive ability of the model comes from the protected attribute, boosting tries to improve performance by using other features and hence, reducing the bias in the final model. For XGB and ADB models, the default number of learners (100) is enough to reach convergence on fairness score. Models TM-XGB2, XGB3 and ADB1, use GridSearch to tune the models and have been assigned very high number of estimators. However, there is no  effect on fairness performance beyond the initial default 100 learners, and is very computationally expensive. On the other hand, GBC models show improvement in fairness when the number of learners are increased beyond. Lastly, our results show that improvement in fairness across boosting rounds does not negatively impact the accuracy, which is interesting given the usual fairness and accuracy trade-off.

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \footnotesize
  \caption{Performance of \textit{AC-ADB1} (AdaBoost) across boosting rounds}
  \renewcommand{\tabcolsep}{1pt}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
          & \textbf{classifier} & \textbf{T0} & \textbf{T10} & \textbf{T20} & \textbf{T30} & \textbf{T40} & \textbf{T50} & \textbf{T60} & \textbf{T70} & \textbf{T80} & \textbf{T90} & \textbf{T99} \\
    \hline
    \textbf{AC} & 0.832 & 0.813 & 0.833 & 0.830 & 0.835 & 0.837 & 0.833 & 0.835 & 0.834 & 0.833 & 0.831 & 0.832 \\
    \hline
    \textbf{F1} & 0.627 & 0.605 & 0.629 & 0.627 & 0.628 & 0.634 & 0.629 & 0.630 & 0.634 & 0.623 & 0.624 & 0.627 \\
    \hline
    \textbf{SPD} & -0.204 & -0.183 & -0.178 & -0.173 & -0.185 & -0.188 & -0.198 & -0.191 & -0.200 & -0.192 & -0.202 & -0.204 \\
    \hline
    \textbf{EOD} & -0.179 & -0.063 & -0.077 & -0.065 & -0.117 & -0.102 & -0.143 & -0.143 & -0.119 & -0.165 & -0.159 & -0.179 \\
    \hline
    \textbf{AOD} & 0.140 & 0.081 & 0.081 & 0.073 & 0.103 & 0.097 & 0.121 & 0.117 & 0.111 & 0.128 & 0.131 & 0.140 \\
    \hline
    \textbf{DI} & -1.310 & -0.960 & -1.075 & -0.980 & -1.176 & -1.180 & -1.253 & -1.202 & -1.239 & -1.247 & -1.289 & -1.310 \\
    \hline
    \textbf{TI} & 0.127 & 0.131 & 0.127 & 0.126 & 0.128 & 0.125 & 0.127 & 0.127 & 0.124 & 0.129 & 0.128 & 0.127 \\
    \hline
    \end{tabular}%
  \label{AC-ADB1}
\end{table}%

%Therefore, the boosting rounds did not have any direct %correlation with the boosting round. To reach this %conclusion, we analyzed different models to investigate %if this could  be attributed to the model type or dataset.

For the other datasets, we did not see substantial improvement or change in fairness performance with more boosting rounds.  Since the datasets are less biased, the weak learners do not derive the majority of the predictive ability from the protected attributes and as boosting is designed to improve accuracy performance, the fairness metrics converge accordingly. In other words, the weak learners do not show the same high level of bias as the models in Titanic. For instance, we analyzed \textit{AC-ADB1} and found that the final fairness performance is worse than if the boosting round had been stopped early, for very similar accuracy performance (accuracy \& f1). Table \ref{AC-ADB1} shows the performance across boosting rounds. 


From the results, we can see that after $10^{th}$ and $20^{th}$ boosting rounds, the model outperforms the final classifier result in both accuracy and fairness metrics. On further inspection, we found that the difference between the predictions of the final classifier and T10 was limited to only 31 instances, all of which were \textit{Females} (protected group) who had been predicted correctly \& positively (\textit{Income} $>$ 50K). Since, boosting was designed to improve performance, the final fairness results can vary. This phenomenon was seen in all the other models and datasets. However,  
this is a very interesting finding because it provides further insight into boosting models and how they can be leveraged to tweak boosting rounds to achieve better fairness while being very accurate. 

\textbf{Bagging}

Compared to boosting models, bagging models exhibit a very different behavior as number of individual learners are increased. For the bagging models (RF,ET) in our benchmark, the results show that a higher number of learners does not have any effect on fairness performance. For all the models across our datasets, we see the number of learners smoothen the performance to avoid extremes. Though this guarantees that the final model is fair than the most biased model, it also interestingly indicates that using high number of trees is computationally expensive and not effective, empirically. To this end, we conclude that the default number of learners (100), adequately satisfy, not only accuracy performance, but also fairness.  \textbf{[Discuss how to represent this result]}

\begin{mdframed}[leftmargin=1cm,
    skipabove=0.2cm,    
    linecolor=white,
    backgroundcolor=gray!5,
    linewidth=2pt,
    roundcorner = 5pt,
    innerleftmargin=1em,
    innerrightmargin=1em,
    innertopmargin=.75em,
    innerbottommargin=.75em,
    %userdefinedwidth=50em,
]
\noindent \textbf{RQ5. What specifications of individual learners can be inferred in different ensemble scenario?}
\end{mdframed}

\textit{\textbf{Stacking}.} We analyze the stacking models for the four datasets in our benchmark. For Titanic ML dataset, we had enough kernels to select the top-6 based on up-votes. However, for other datasets there were few to no stacking model kernels available. For these datasets, we used the top-voted kernel with multiple models to build a stacking model using the various types of ML models in the kernel. This ensures that our results are consistent across datasets and account for variability in datasets.

Stacking uses a two-level learning method to improve model performance by stacking the first-level individual learner's  and inputting their output  to the second-level meta-learner (default: Logistic Regression in scikit-learn) to generate predictions \cite{WOLPERT1992241}. We analyze the stacking models by generating fairness results not only for the final ensemble model, but also for the chain of individual estimators that are part of the first-level models.

\textbf{\textit{Analysis.}} 

\textit{Two-layered estimators improve fairness.} All of the Titanic ML stacking models shown in Figure \ref{stacking:comparison} exhibit similar bias except \textit{TM-STK5}, which is the least biased model for the Titanic ML dataset for all fairness metric except Thiel Index (TI). On closer inspection, we found out that \textit{TM-STK5} uses a two-layered stacking approach where the second layer of the individual estimators, act as the meta-learner for the first layer:

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}
\lstset{style=mystyle}

\begin{lstlisting}[language=Python]
layer_one_estimators = [('rf_1', RandomForestClassifier(n_estimators=40, random_state=42)),('knn_1', KNeighborsClassifier(n_neighbors=6))]
layer_two_estimators = [('rf_2', RandomForestClassifier(n_estimators=40, random_state=42)),('xg_2', XGBClassifier(objective = 'binary:logistic', colsample_bytree = 0.8, learning_rate = 0.3, max_depth = 7, min_child_weight = 3, n_estimators = 100, subsample = 0.6))]
layer_two = StackingClassifier(estimators=layer_one_estimators, final_estimator=XGBClassifier(n_estimators  = 100))
model =  StackingClassifier(estimators=layer_one_estimators, final_estimator=layer_two)}
\end{lstlisting}

We investigated why this particular model performed significantly better in fairness terms by comparing it to other kernels for the Titanic ML dataset. We found that the difference in feature set or the combination of individual learners was not responsible, rather the better fairness performance is attributed to the two-layered nested stacking approach.

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[!htbp]
  \centering
  {\footnotesize 
  %\renewcommand{\tabcolsep}{1pt}
  \caption{\textbf{Fairness metrics of the models using single vs nested-layer stacking}}
  \label{tab:Nested_Stacking}%
 \resizebox{\columnwidth}{!}{   \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{\textbf{Models}} & \multicolumn{7}{c|}{\textbf{Single-layer Stacking}}   & \multicolumn{7}{c|}{\cellcolor[HTML]{EBEBEB}\textbf{Nested-layer Stacking}} \\
\cline{2-15}          & \multicolumn{1}{l|}{\textbf{Acc}} & \multicolumn{1}{l|}{\textbf{F1}} & \multicolumn{1}{l|}{\textbf{SPD}} & \multicolumn{1}{l|}{\textbf{EOD}} & \multicolumn{1}{l|}{\textbf{AOD}} & \multicolumn{1}{l|}{\textbf{DI}} & \multicolumn{1}{l|}{\textbf{TI}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EBEBEB}\textbf{Acc}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}\textbf{F1}}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}\textbf{SPD}}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}\textbf{EOD}}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}\textbf{AOD}}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}\textbf{DI}}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}\textbf{TI}}} \\ 
    \hline
    \multicolumn{1}{|l|}{TM-STK1} & 0.802 & 0.741 & -0.717 & -0.639 & 0.554 & -2.407 & 0.178 & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.765} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.701} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-0.697} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-0.613} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.598} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-2.071} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.196} \\
    \hline
    \multicolumn{1}{|l|}{TM-STK2} & 0.847 & 0.800 & -0.843 & -0.720 & 0.675 & -2.642 & 0.114 & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.728} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.660} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-0.454} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-0.392} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000} 0.300} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-1.152} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.209} \\
    \hline
    \multicolumn{1}{|l|}{TM-STK3} & 0.836 & 0.753 & -0.773 & -0.617 & 0.610 & -2.398 & 0.117 & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.772} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.630} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-0.488} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-0.367} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.347} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-1.612} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.184} \\
    \hline
    \multicolumn{1}{|l|}{TM-STK4} & 0.828 & 0.763 & -0.781 & -0.623 & 0.625 & -2.468 & 0.113 & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.757} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.663} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-0.486} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-0.480} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.349} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-1.305} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.163} \\
    \hline
    \multicolumn{1}{|l|}{TM-STK6} & 0.877 & 0.836 & -0.756 & -0.645 & 0.504 & -2.315 & 0.096 & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.836} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.790} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-0.542} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-0.356} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.255} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-1.329} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.111} \\
    \hline
    AC-STK1 & 0.853 & 0.662 & -0.184 & -0.103 & 0.090 & -1.289 & 0.122 & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.809} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.532} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-0.104} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-0.009} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.022} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-0.737} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.165} \\
    \hline
    BM-STK1 & 0.910 & 0.549 & 0.123 & 0.095 & 0.078 & 0.895 & 0.070 & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.896} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.430} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.101} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-0.007} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.046} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.901} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.087} \\
    \hline
    GC-STK1 & 0.680 & 0.342 & -0.126 & -0.045 & 0.142 & -0.152 & 0.115 & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.627} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.423} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-0.074} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-0.121} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.074} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}-0.108} & \cellcolor[HTML]{EBEBEB}{\color[HTML]{000000}0.233} \\
    \hline
    \end{tabular}}}%
\end{table}%


We validated our findings by training all of the stacking based kernels in our benchmark on this 2-layered nested stacking model. To ensure consistency, we did not change the feature set or any preprocessing method for any kernel. The results are shown in Table \ref{tab:Nested_Stacking}. For all stacking models across the four datasets in our benchmark, every model significantly improved in all fairness measures while not affecting accuracy measures drastically. For example, \textit{TM-STK6} improved \textbf{Statistical Parity Difference} (SPD) scores by $28\%$ while only accuracy dropping $4.68\%$. Overall across all datasets, the accuracy score dropped by $6.50\%$ while the SPD improved by $31.8\%$. Two-layered nested stacking approach improves fairness scores dramatically due to the addtion of a second-layer of ensembles that act as a meta-learner. Stacking generalization works by first estimating the error of the generalizer and then using a second classifier (meta-learner) to \textit{correct} the errors i.e. whose output is the final prediction \cite{WOLPERT1992241}. In two-layered stacking, the first layer uses a list of estimators (ensembles) to generate a set of predictions for each of the estimators, instead of using a single classifer (meta-learner), the predictions are fed into another set of estimators. This ensures that a single meta-learner does not entirely predict the final outcome based on the first-level errors. Rather the nested ensembles create a new set of predictions which are then finally inputted into the final meta-classifier of the second layer. The introduction of a second-layer of ensembles guarantees that the final fairness metrics will be better than the most biased single classifier \cite{Nina}.



\textit{Default meta-learner optimized for accuracy.} The default meta-learner for stacking models in Sklearn is logistic regression. Our results show that while the accuracy of the models are better with logistic regression as the meta-learner, it introduces significant bias in the final predictions. We analyze all the models that use \textit{LogisticRegression()}: \textit{TM-STK2, TM-STK4, TM-STK6, AC-STK1, BM-STK1, GC-STK1}. For all these models, we use XGBoost as the meta-learner instead, as an example of an ensemble method that performs equally well but is less biased. Our results did not significantly vary between the use of other ensembles as the final estimator. The change in performance and total bias (sum of the absolute values of bias) is depicted in Figure \ref{stacking:comparison}. As we can see, the total bias is reduced for all the stacking models in our benchmark while there is very minimal change in accuracy scores. The maximum change in performance for any of the model is less than 0.1 (GC-STK). Therefore, the use of an ensemble as a final estimator can improve fairness of stacking models.

\begin{figure}[!htbp]
  \centering

    \includegraphics[scale=0.4]{Figures/Finding2_stacking.pdf}
    \caption{Change of performance and total bias when using XGBoost Classifier as meta-learner in Stacking (negative value denotes reduction}
    \label{stacking:comparison}
\end{figure}




%\begin{figure}
%%\centering
%\begin{minipage}{.5\textwidth}
%  \centering
 % \includegraphics[width=\linewidth]{Figures/chart.pdf}
  %\captionof{figure}{A figure}
  %\label{fig:test1}
%end{minipage}%
%%\begin{minipage}{.4\textwidth}
  %\centering
  %\includegraphics[width=\linewidth]{Figures/chart.pdf}
  %\captionof{figure}{Another figure}
  %\label{fig:test2}
%\end{minipage}
%\end{figure}


\textbf{AdaBoost.}

\lstset{style=mystyle}

\begin{lstlisting}[language=Python]
model = AdaBoostClassifier(DecisionTreeClassifier())
model = AdaBoostClassifier(base_estimator = DecisionTreeClassifier(criterion = 'entropy'), learning_rate = 0.3, random_state = 7)
\end{lstlisting}

\textbf{Analysis.}

\textit{Decision stumps vs deep trees.} The default base estimator for AdaBoost is a decision tree classifier with \textit{max depth = 1}, also called a decision stump. Decision stump is a decision tree with only 1 split, which is usually the best split based on the training features. In our benchmark, \textit{AC-ADB2} and \textit{TM-ADB1} were the only two models that did not use the default decision stump. To investigate the effect of using a decision stump with a full-grown tree on fairness, we compare the performance of both of these models using these two methods. As shown in \ref{Fig:decision vs stump}, we see similar behavior to what we saw as boosting rounds progressed. For highly biased dataset like Titanic, decision stumps worsen the behavior as the weak learner is primarily composed of the protected attribute due to it's higher predictive power. However, the opposite is seen in AC-ADB2 because deeper trees are more complex and will add bias by using the predictive power in the protected attribute, which is not present in it's weak learner

\begin{figure}[!htbp]
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{Figures/chart-2.pdf}
  \label{fig:test1}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{Figures/chart_1.pdf}
  \label{fig:test2}
\end{minipage}
\caption{Percentage change in performance using Decision Stump AC-ADB2 and TM-ADB1}
\label{Fig:decision vs stump}
\end{figure}



\begin{figure}[htbp]
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{Figures/TM_RandomSplit.pdf}
  \label{fig:test1}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{Figures/AC_RandomSplit.pdf}
  \label{fig:test2}
\end{minipage}
\caption{Percentage change in performance using Decision Stump AC-ADB2 and TM-ADB1}
\label{Fig:decision vs stump}
\end{figure}

\begin{mdframed}[leftmargin=1cm,
    skipabove=0.2cm,    
    linecolor=white,
    backgroundcolor=gray!5,
    linewidth=2pt,
    roundcorner = 5pt,
    innerleftmargin=1em,
    innerrightmargin=1em,
    innertopmargin=.75em,
    innerbottommargin=.75em,
    %userdefinedwidth=50em,
]
\noindent \textbf{RQ6. How the fairness composition in ensemble be leveraged towards building fairer models?}
\end{mdframed}

In this RQ, we investigate how we can use the composition methods to build fairer models...

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> background.tex <==
\section{Background and Motivation}
\label{background}

%\hridesh{Can you make this section Background and Motivation? Perhaps there is StackOverflow post or something that motivates your study...}
In this section, we first discuss fairness in ML software and some terminologies. Next, we present an ensemble to show that ensemble design affects the fairness of the model and the need to study bias induced by certain ensemble parameters.

%\subsection{Fairness in ML software}
%\label{subsec:fairness-in-ml}

% Table generated by Excel2LaTeX from sheet 'hierarchy'
\begin{table*}[!htbp]
  \centering
  \footnotesize
  \renewcommand{\tabcolsep}{1pt}
  
  \caption{Ensemble types used in our experiments}
   \begin{tabular}{c|c|m{6.5cm}|c|c}
    \hline 
    \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Categories}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Ensemble Types}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Algorithms}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Composition}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Classifiers}} \\
    \hline 
    \multirow{3}{*}{Sequential} & \multirow{3}{*}{Boosting} & \multirow{3}{*}{\shortstack {Construct n homogeneous estimators sequentially that 
    \\ improve predictions based on the previous estimator's 
    \\ incorrect predictions}} & Homogeneous & XGBoost \\
          &       &       & Homogeneous & AdaBoost \\
          &       &       & Homogeneous & Gradient Boosting \\
    \hline
    \multirow{5}{*}{Parallel} & \multirow{3}{*}{Bagging} & \multirow{3}{*}{\shortstack{Construct \textit{n} parallel homogeneous models that are
    \\ aggregated using averaging}} & Homogeneous & Random Forest \\
         &       &       & Homogeneous & ExtraTrees \\
         &       &       & Homogeneous & Bagging Classifier \\
\cline{2-5}          & Voting & Construct a list of n hetereogeneous user-specified weighted classifiers that are aggregated using majority voting or argmax & Heterogeneous & Voting Classifier \\
\cline{2-5}          & Stacking & Construct a list of n hetereogeneous classifiers as base learners and a meta-classifier to decide weights for each learner & Heterogeneous & Stacking Classifier \\
    \hline
    \end{tabular}%
  \label{tab:ensemble-types}%
\end{table*}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \scriptsize
  \renewcommand{\tabcolsep}{1pt}
  \caption{Summary of the datasets and the number of models collected for each in the benchmark }
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \hline
    \cellcolor[HTML]{C0C0C0}\textbf{Datasets} & \cellcolor[HTML]{C0C0C0}\textbf{PA} &
    \cellcolor[HTML]{C0C0C0}\textbf{Size} &
    \cellcolor[HTML]{C0C0C0}\textbf{\# XGB} & \cellcolor[HTML]{C0C0C0}\textbf{\# ADB} & \cellcolor[HTML]{C0C0C0}\textbf{\# GBC} & \cellcolor[HTML]{C0C0C0}\textbf{\# RF} & \cellcolor[HTML]{C0C0C0}\textbf{\# ET} & \cellcolor[HTML]{C0C0C0}\textbf{\# STK} & \cellcolor[HTML]{C0C0C0}\textbf{\# VT} & \cellcolor[HTML]{C0C0C0}\textbf{Total} \\
    \hline
    \cellcolor[HTML]{EDEDED}\textbf{Adult Census} & \cellcolor[HTML]{EDEDED} sex &
    \cellcolor[HTML]{EDEDED} 32561 &
    \cellcolor[HTML]{EDEDED} 6     & \cellcolor[HTML]{EDEDED} 6     &  \cellcolor[HTML]{EDEDED} 6     & \cellcolor[HTML]{EDEDED} 6     &  \cellcolor[HTML]{EDEDED} 6     &  \cellcolor[HTML]{EDEDED} 1     & \cellcolor[HTML]{EDEDED} 2     & \cellcolor[HTML]{EDEDED} 33 \\
    \textbf{Titanic ML} & sex  
    & 891 & 6     & 6     & 6     & 6     & 6     & 6     & 6     & 42 \\
    \cellcolor[HTML]{EDEDED}\textbf{Bank Marketing} & \cellcolor[HTML]{EDEDED} age   &
    \cellcolor[HTML]{EDEDED} 41118 &
    \cellcolor[HTML]{EDEDED} 6     & \cellcolor[HTML]{EDEDED} 6     & \cellcolor[HTML]{EDEDED} 6     & \cellcolor[HTML]{EDEDED} 6     & \cellcolor[HTML]{EDEDED} 2     &  \cellcolor[HTML]{EDEDED} 1     & \cellcolor[HTML]{EDEDED} 2     & \cellcolor[HTML]{EDEDED} 29 \\
    \textbf{German Credit} & sex   & 1000 & 6     & 1     & 1     & 6     & 1     & 1     & 1     & 17 \\
    \hline
    \end{tabular}%
  \label{tab:datasetsummary}%
  \begin{tablenotes}
      \small
      \centering
      \item  XGB: XGBoost, ADB: AdaBoost, GBC: Gradient Boosting
      , RF: Random Forest, ET: Extra Trees, STK: Stacking, VT: Voting
    \end{tablenotes}
\end{table}%

%Data-driven software has been widely adopted in modern society, with reported implications for disadvantaged minority groups \cite{mattu_machine_nodate, KHANDANI20102767}. Fairness-aware machine learning addresses predictive models discriminating against people based on their \textit{protected attributes} such as race, sex, etc. %Previous work identified the protected attributes of interest in ML predictive tasks \cite{10.1145/3287560.3287594}. 
%One trivial idea is to train the model without the protected attribute. However, it fails to account for the correlation of protected attributes with other attributes \cite{10.1145/1401890.1401959}. 
%This has increased interest in developing algorithms to mitigate algorithmic bias. Several fairness metrics have been proposed to measure the bias quantitatively, broadly divided into two categories. \textit{Group fairness} means similar predictive outcomes on a group level for protected attributes, e.g., race (Asian/White). \textit{Individual fairness} determines that similar predictive outcomes go to similar individuals \cite{10.1145/2090236.2090255}. We consider binary classification problems in fairness where a class label is denoted as \textit{favorable} if it gives an advantage to a group (\textit{privileged}) or individual and vice-versa e.g. loan approval. The subset of fairness metrics used in this study have been described in \S \ref{subsubsec:fairness-measures}.

%\begin{itemize}
%\item  \textit{Group fairness} means similar predictive outcomes on a group level for protected attributes, e.g., race (Asian/White)
%\item \textit{Individual fairness} determines that similar predictive outcomes go to similar individuals \cite{10.1145/2090236.2090255}
%\end{itemize}
%We consider binary classification problems in fairness where a class label is denoted as \textit{favorable} if it gives an advantage to a group (\textit{privileged}) or individual and vice-versa e.g., loan approval. The subset of fairness metrics used in this study have been described in \S \ref{subsubsec:fairness-measures}.
%the composition of fairness and the effect of ensemble-specific hyperparameters in ensembles on fairness mitigation. This study explores the fairness properties of ensembles and it's learners.}


\subsection{Ensemble learning in ML software}
\label{subsec:ensemble-in-ml}
{\em Ensemble models} are a class of ML classifiers where the predictions from different learners (models) are pooled using a combination method (voting, average, random, etc.) to make the final predictions. %\hridesh{The previous sentence is an example of what you need earlier in the abstract and intro} 
%\hridesh{You are NOT YET DONE convincing SE reviewers that studying ensemble is important, you need to do a little more selling here again about why these kinds of models are important to study.}
\textcolor{blue}{Ensemble models are the most mentioned ML/DL algorithms on Kaggle \cite{DBLP:journals/corr/abs-2006-08334} and are widely used due to their superior performances in ML challenges \cite{10.5555/2627435.2697065, inproceedings-OnlineLearning, dietterich2000experimental, bauer1999empirical, HOSNI201989}. Out of the top models on Kaggle for popular fairness datasets used by previous SE researchers, ensemble models comprise more than $80\%$ of the total models \cite{10.1145/3368089.3409704,10.1145/3468264.3468536}. Just like traditional ML models, we observe that ensembles also suffer from fairness issues. Categories of ensembles are based on homogeneity, learning technique, and ensemble types. All the ensemble types covered in our study and the corresponding classifiers are given in Table \ref{tab:ensemble-types}. There are mainly two categories of ensemble models: Sequential and Parallel.}

\textbf{\textit{Sequential Ensembles.}} These ensembles sequentially generate base learners. Each learner in the ensemble depends on the previous learners in the sequence because the next learner attempts to correct the wrong predictions from the previous learner and so on \cite{8360836}. AdaBoost is an example of a sequential model where it reweighs (higher) misclassified examples.

%\begin{figure}[]
%\includegraphics[width=1\linewidth]{Figures/Benchmark-Collection.pdf}
%\caption{\textbf{Benchmark collection process}}
%\label{benchmark}
%\vspace{-4mm}
%\end{figure}

\textbf{\textit{Parallel Ensembles.}} Parallel ensembles train individual base learners in parallel and independently of each other. A random subset of training data is used to construct these learners and combined using techniques such as bagging or voting, which encourages improved variance \cite{8360836} e.g., Random Forest.

\textit{\textbf{Homogeneity of ensembles.}}
Ensemble methods that use single-type base learners are called \textit{homogeneous} models \cite{Elish2013EmpiricalSO}. These individual learners are combined to generate the final result, e.g., {\em XGBoost} and {\em AdaBoost} use decision trees. By contrast, \textit{heterogeneous} ensembles combine the predictions of dissimilar individual learners \cite{Elish2013EmpiricalSO}. A popular heterogeneous ensemble method is {\em Voting}. Finally, ensemble method types are divided into {\em Boosting, Bagging, Voting}, \& {\em Stacking} \cite{scikit-learn}.

\textcolor{blue}{In this paper, we use the term {\em ensemble parameters} to mean hyperparameters like \textit{number of learners}, \textit{combination methods}, etc., that dictate how ensembles combine base learners and hence affect ensemble fairness \& design (Table \ref{Parameters}).}

\subsection{Motivation}
\textcolor{blue}{Unlike traditional software, data-driven software takes input data, performs pre-processing, and applies an ML algorithm with tuned hyperparameters to build a rule-based logic that a developer does not write manually. These hyperparameters are tuned for accuracy and have been shown to encode bias \cite{}. However, no work has studied the composition of fairness in ensembles and the bias induced by \textit{ensemble hyperparameters}. In this study, we postulate that the ensembles can be designed to be fairer without using any mitigation techniques and explore fairness composition to design fair ensembles software.}

%\hridesh{Summary: You are not done selling your work to SE reviewers yet, and this section should be revised in light of that. If they don't buy the motivation, they will find 50 reasons to reject your paper even if it is an immaculate piece of work.}

%\textit{1) Boosting.} Boosting is a sequential ensemble technique that learns from previous learners in the sequence to correctly predict the incorrect predictions in the next round \cite{Schapire02theboosting}. In the case of AdaBoost, it achieves this by giving a higher weight to incorrectly predicted data in the next learner. All of the boosting methods are homogeneous.

%\textit{2) Bagging.} Bagging is the combination of Bootstrapping and Aggregation. Bootstrap is a sample with a replacement technique \cite{10.2307/2958830}, whereas aggregation refers to combining the results of each learner to aggregate the predictions. In Bagging, weak learners are combined in parallel to construct a strong learner with less variance and hence, less prone to overfitting \cite{breiman96}. Bagging examples include ExtraTrees and Random Forests.

%\textit{3) Stacking.} Stacking or \textit{stacked generalization} is an ensemble method that combines the predictions of multiple classifiers using a meta-learner \cite{WOLPERT1992241}. The first-level models are a list of ML models constructed in parallel using a train and validation dataset. The predictions from these individual learners are then passed to the meta-learner as new features. The meta-learner uses the list of individual models to predict the final result, which usually performs better than the individual first-level models. Stacking can handle both homogeneous and heterogeneous sets of first-level models.

%\textit{4) Voting.} Voting is an ensemble method where the predicted class is either the one with majority number of votes (hard) or the max of the probability (soft) from weighted classifiers in the ensemble \cite{10.5555/3327144.3327272}. Voting can also handle both homogeneous and heterogeneous classifiers

==> fairness-guarantee.tex <==


\section{Fairness Guarantees in Ensemble}
\label{sec:fairness-guarantee}

In \S 4, we analyzed the composition of fairness in heterogeneous models which combine the powers of each individual learner to aggregate fairness scores. \citeauthor{Nina} first presented theoretical evidence of an ensemble of random selection based classifiers being fair \cite{Nina}. More recent works provided empirical evidence and built upon this by arguing that the ensemble is guaranteed to be at least as fair as the most biased classifier in the ensemble \cite{8995403, 9462068}. However, these observations were limited to bagging and random selection strategy only. In this section, we explore whether heterogeneous learners guaranteed to outperform their individual learners \textbf{(RQ2)} and provide empirical evidence to the contrary.

We explore this for both stacking and voting and find that this is not always true. For example, TM-VC5 is a soft voting ensemble with 3 classifiers \textit{Logistic Regression (LR)}, \textit{Random Forest (RF)} and \textit{AdaBoost (ADB)}. The results for these individual classifiers along with it's ensemble are reported in Table \ref{Voting-Guarantee}. We can see that in terms of \textit{SPD} and \textit{AOD}, the Voting ensemble actually performs worse than the most biased individual classifiers (\textit{LR} in this case). Recall from earlier that soft-voting takes the average of the probabilities for each class label (with the higher winning). Upon further investigation, we find that that the ensemble has outperformed its individual classifiers, in terms of accuracy. In other words, this suggests that the number of correct but \textit{biased} predictions in the ensemble increases. Therefore, this shows that classifiers of voting ensembles can combine in a way that can worsen the fairness performance of the ensemble for specific metrics.

Similarly, we see that stacking is not guaranteed to outperform  e.g. AC-STK1. As illustrated in Table \ref{Voting-Guarantee}, AC-ST1 has 5 estimators \textit{ExtraTrees (ET), Gradient Boosting Classifier (GBC), Random Forest (RF), XGBoost (XGB) and Light Gradient Boosting (LGBM)}. We can see that the final stacking \textit{SPD} score is slightly worse than \textbf{GBC}, which is the most biased estimator in stacking. We do note that the difference here is insignificant, however, it provides empirical evidence of existence of combination that can potentially result in a more biased ensemble.

% Table generated by Excel2LaTeX from sheet 'AC-STK1'
\begin{table}[t]
  \centering
  \footnotesize
%\renewcommand{\tabcolsep}{1pt}
%  \vspace{-2mm}
 \caption{Comparison of fairness performance between individual classifiers and final voting \& stacking classifiers. For SPD and AOD, TM-VT5 is more bias than LR while AC-STK1 is more unbiased than GBC  (worst learners in each ensembles)}
%  \vspace{-2mm}
\resizebox{\columnwidth}{!}{   
    \begin{tabular}{|c|c|cccccc|}
    \hline
    \multirow{8}{*}{\rotatebox[origin=c]{90}{TM-VT5}} &  & {\textbf{LR}} & \textbf{RF} & \textbf{ADB} & \textbf{Voting} &       &  \\ \hline
          & \textbf{Acc} & 0.795 & 0.787 & 0.761 & 0.810 &       &  \\
          & \textbf{F1} & 0.718 & 0.698 & 0.686 & 0.738 &       &  \\
          & \textbf{SPD} & -0.751 & -0.729 & -0.722 & -0.772 &       &  \\
          & \textbf{EOD} & -0.671 & -0.671 & -0.671 & -0.625 &       &  \\
          & \textbf{AOD} & 0.628 & 0.614 & 0.621 & 0.629 &       &  \\
          & \textbf{DI} & -2.074 & -2.146 & -1.773 & -2.099 &       &  \\
          & \textbf{TI} & 0.137 & 0.148 & 0.144 & 0.124 &       &  \\
          \hline \hline
     \multirow{8}{*}{\rotatebox[origin=c]{90}{AC-STK1}} &  & \textbf{ET} & \textbf{GBC} & {\textbf{RF}} & {\textbf{XGB}} & {\textbf{LGBM}} & \textbf{Stacking} \\ \hline
          & \textbf{Acc} & 0.842 & 0.853 & 0.842 & 0.851 & 0.851 & 0.853 \\
          & \textbf{F1} & 0.641 & 0.661 & 0.648 & 0.660 & 0.661 & 0.662 \\
          & \textbf{SPD} & -0.153 & -0.183 & -0.161 & -0.175 & -0.182 & -0.184 \\
          & \textbf{EOD} & -0.020 & -0.108 & -0.030 & -0.074 & -0.098 & -0.103 \\
          & \textbf{AOD} & 0.040 & 0.092 & 0.048 & 0.073 & 0.087 & 0.090 \\
          & \textbf{DI} & -0.961 & -1.302 & -0.976 & -1.166 & -1.235 & -1.289 \\
          & \textbf{TI} & 0.128 & 0.122 & 0.124 & 0.122 & 0.121 & 0.122 \\
          \hline
    \end{tabular}}%
  \label{Voting-Guarantee}%
  \vspace{-4mm}
\end{table}%

Overall, our empirical evaluation of heterogeneous models with stacking and voting show that they perform comparably (at best) to the worst classifier in the ensemble but are not necessarily guaranteed to outperform the most biased classifier in terms of fairness. To reduce the possibility of this, developers should add more number of classifiers, especially in soft voting, where a highly biased classifier can skew the final result negatively. This is discussed further in detail in \S \ref{sec:fair-design}.




==> measures.tex <==
\section{Measures}
\label{measures}

Multiple quantitative fairness and accuracy measures are available to evaluate a model. However, we only focus on the measures that have been previously used in literature \cite{10.1145/3287560.3287589, 10.1145/3368089.3409704}, as they  provide a good representation of metrics. Let $D = (T,S,Y)$ be a dataset where $D$ is the portion of the dataset used for training, $S$ is the protected attribute ($S = 1$, if privileged group, otherwise $S = 0$) and $Y$ is the classification label ($Y = 1$ denotes favorable label, otherwise $Y = 0$). Let $\hat{Y}$ denote the prediction of an ML model. Next, we define our measures in terms of these notations.

\subsection{Accuracy Measures}

We evaluate the performance of the models using standard accuracy measures for comparison across datasets and relationship with fairness. For accuracy measures, we use the following two accuracy metrics:

\textit{Accuracy.} To evaluate the overall performance of the model, we use the accuracy measure, $P[\hat{Y} = Y]$.
\begin{center}
    Accuracy = $\frac{(TP+TN)}{TP+TN+FP+FN}$
\end{center}
    
 
\textit{F1 Score.} To evaluate the performance of the model in relation to both recall and precision, we use the F1 score which is the harmonic mean of precision and recall.

\begin{center}
    F1 = 2 *(Precision * Recall)/Precision + recall)
\end{center}

where Recall = $TP/(TP + FN)$, Precision $ = TP/(TP+FP)$

\subsection{Fairness Measures}

Broadly, fairness metrics are divided into three different categories, and multiple fairness metrics have been proposed in literature \cite{Binns2018FairnessIM}. We have selected a subset of these metrics that are representative of the three categories without being exhaustive. Furthermore, we have followed the recommendations of Friedler \textit{et al.} \cite{10.1145/3368089.3409704} in terms of metrics selection.

\textbf{Group fairness metrics:} \\

\paragraph{Equal Opportunity Difference (EOD):} This is defined by the difference in true-positive rates (TPR) between privileged and unprivileged groups.

\begin{center}
    $EOD = TPR_{up} - TPR_p$
\end{center}
where $TPR = TP/(TP + FN), FPR = FP/(FP + TN)$  \\

\textit{Average Odds Difference (AOD):} This is defined by the mean of false-positive rate (FPR) difference and true-positive rate difference between unprivileged and privileged groups. \cite{NIPS2016_9d268236}

\begin{center}
    $AOD = {(FPR_{up} - FPR_p) + (TPR_{up} - TPR_p)}/2$
\end{center} 

\paragraph{Disparate Impact (DI):} This is defined as the ratio of the probability of unprivileged group getting a favorable prediction and the probability of privileged group getting a favorable prediction \cite{JMLR:v20:18-262}

\begin{center}
    $DI = P[\hat{S} = 1| Y = 0]/ P[\hat{S} = 1| Y = 1]$
\end{center} 

To improve readability when comparing different metrics in the same table, we convert Disparate Impact (DI) to log scale.

\paragraph{Statistical Parity Difference (SPD):} This is defined similarly to DI, but in this case, we use a difference between the probabilities \cite{Calders2010ThreeNB}.

\begin{center}
    $SPD = P[\hat{S} = 1| Y = 0] - P[\hat{S} = 1| Y = 1]$
\end{center}

\subsubsection{Individual fairness metrics:}

\paragraph{Theil Index (TI):} Theil Index measures both the group and individual fairness \cite{10.1145/3219819.3220046}. It is defined using the following equation where $b_i = \hat{s}_i - s_i + 1$

\[   TI = \sum_{i=1}^{n} \frac{b_i}{\Bar{a}} ln \frac{b_i}{\Bar{a}}\]


